Planetary formation and water delivery in the habitable zone around solar-type stars in different dynamical environments

Aims. We study the formation and water delivery of planets in the habitable zone (HZ) around solar-type stars. In particular, we study different dynamical environments that are defined by the most massive body in the system. Methods. First of all, a semi-analytical model was used to define the mass of the protoplanetary disks that produce each of the five dynamical scenarios of our research. Then, we made use of the same semi-analytical model to describe the evolution of embryos and planetesimals during the gaseous phase. Finally, we carried out N-body simulations of planetary accretion in order to analyze the formation and water delivery of planets in the HZ in the different dynamical environments. Results. Water worlds are efficiently formed in the HZ in different dynamical scenarios. In systems with a giant planet analog to Jupiter or Saturn around the snow line, super-Earths tend to migrate into the HZ from outside the snow line as a result of interactions with other embryos and accrete water only during the gaseous phase. In systems without giant planets, Earths and super-Earths with high water by mass contents can either be formed in situ in the HZ or migrate into it from outer regions, and water can be accreted during the gaseous phase and in collisions with water-rich embryos and planetesimals. Conclusions. The formation of planets in the HZ with very high water by mass contents seems to be a common process around Sun- like stars. Our research suggests that such planets are still very efficiently produced in different dynamical environments. Moreover, our study indicates that the formation of planets in the HZ with masses and water contents similar to those of Earth seems to be a rare process around solar-type stars in the systems under consideration.

==> Graficos/Jupiter/fixbb <==
#!/bin/bash

# This is fixbb version 0.31.  Copyright 2000 by Jeff Spirko.
# Redistributable under the GNU General Public License.
# See http://topquark.dhs.org/~spirko/fixbb/

# Changes by Petr Mikulik:
#   -  8.  9. 2000: working file in the $TMP directory; remove backup file
#   - 18. 10. 2000: AWKPARSEBB to support multiple-page (non-EPS) documents
#   - 26. 10. 2000: error if bounding box not determined (GS < 5.50 or empty
#     pages); page status info added

# Options for ghostscript to print the BoundingBox without other junk.
GSOPTS="-dQUIET -dBATCH -dNOPAUSE -sDEVICE=bbox"
export GSOPTS

# Original awk program, checks each line of the file
#AWKPROG='{ if ($1 == "%%BoundingBox:") 
#  print $1, ENVIRON["bbox"]; 
#  else print;}'

# Slightly faster version, doesn't bother looking after finding a BoundingBox.
# What happens if there is more than one BoundingBox?  Can this happen?
AWKPROG='
	(found) { print; next }
	$1 == "%%BoundingBox:" { print $1, ENVIRON["bbox"]; found=1; next }
	{ print }
	'

# Finds min and max of the 4 numbers after the "%%BoundingBox:" label
AWKPARSEBB='
	BEGIN { x1=99999; y1=99999; x2=0; y2=0; page=0 }
	$1!= "%%BoundingBox:" { next }
	$2<0 || $3<0 { next }
	x1>$2 { x1=$2 }
	y1>$3 { y1=$3 }
	x2<$4 { x2=$4 }
	y2<$5 { y2=$5 }
	{ page++; printf "Page " page ": " $0 "  max = " x1 " " y1 " " x2 " " y2  "  \t\r" >"/dev/stderr" }
	END { printf "\t\t\t\t\t\t\t\r" >"/dev/stderr"
	      print x1 " " y1 " " x2 " " y2 }
	'

export bbox

# Each command-line argument is assumed to be a file to process
for FILE in $* ; do

#  BAK=${FILE}~
#  if [ "$TMP" = "" ]; then TMP="."; fi; BAK=$TMP\fixbb__.ps
  BAK='fixbb$$.ps'

  # Get the correct BoundingBox from ghostscript.
  # Old: bbox=`gs ${GSOPTS} ${FILE} 2>&1 | gsort | head -1 | cut -d\  -f 2-`
  bbox=`/usr/bin/gs ${GSOPTS} ${FILE} 2>&1 | awk "$AWKPARSEBB"`

  case $bbox in
    "99999 99999 0 0")
	echo "Bounding box was NOT determined (empty pages or Ghostscript >= 5.50 required)"
	exit ;;
  esac

  echo "Bounding box for \""$FILE"\" is: "$bbox

  # Save the old version of the file
  mv $FILE $BAK

  # Create the new version, replacing the old BoundingBox
  awk "$AWKPROG" $BAK > $FILE

  case `uname` in 
    "OS/2") dos2unix $FILE ;;
  esac

  # delete the backup file
  rm -f $BAK

done


==> Graficos/SuperTierraI/Snapshots/fixbb <==
#!/bin/bash

# This is fixbb version 0.31.  Copyright 2000 by Jeff Spirko.
# Redistributable under the GNU General Public License.
# See http://topquark.dhs.org/~spirko/fixbb/

# Changes by Petr Mikulik:
#   -  8.  9. 2000: working file in the $TMP directory; remove backup file
#   - 18. 10. 2000: AWKPARSEBB to support multiple-page (non-EPS) documents
#   - 26. 10. 2000: error if bounding box not determined (GS < 5.50 or empty
#     pages); page status info added

# Options for ghostscript to print the BoundingBox without other junk.
GSOPTS="-dQUIET -dBATCH -dNOPAUSE -sDEVICE=bbox"
export GSOPTS

# Original awk program, checks each line of the file
#AWKPROG='{ if ($1 == "%%BoundingBox:") 
#  print $1, ENVIRON["bbox"]; 
#  else print;}'

# Slightly faster version, doesn't bother looking after finding a BoundingBox.
# What happens if there is more than one BoundingBox?  Can this happen?
AWKPROG='
	(found) { print; next }
	$1 == "%%BoundingBox:" { print $1, ENVIRON["bbox"]; found=1; next }
	{ print }
	'

# Finds min and max of the 4 numbers after the "%%BoundingBox:" label
AWKPARSEBB='
	BEGIN { x1=99999; y1=99999; x2=0; y2=0; page=0 }
	$1!= "%%BoundingBox:" { next }
	$2<0 || $3<0 { next }
	x1>$2 { x1=$2 }
	y1>$3 { y1=$3 }
	x2<$4 { x2=$4 }
	y2<$5 { y2=$5 }
	{ page++; printf "Page " page ": " $0 "  max = " x1 " " y1 " " x2 " " y2  "  \t\r" >"/dev/stderr" }
	END { printf "\t\t\t\t\t\t\t\r" >"/dev/stderr"
	      print x1 " " y1 " " x2 " " y2 }
	'

export bbox

# Each command-line argument is assumed to be a file to process
for FILE in $* ; do

#  BAK=${FILE}~
#  if [ "$TMP" = "" ]; then TMP="."; fi; BAK=$TMP\fixbb__.ps
  BAK='fixbb$$.ps'

  # Get the correct BoundingBox from ghostscript.
  # Old: bbox=`gs ${GSOPTS} ${FILE} 2>&1 | gsort | head -1 | cut -d\  -f 2-`
  bbox=`/usr/bin/gs ${GSOPTS} ${FILE} 2>&1 | awk "$AWKPARSEBB"`

  case $bbox in
    "99999 99999 0 0")
	echo "Bounding box was NOT determined (empty pages or Ghostscript >= 5.50 required)"
	exit ;;
  esac

  echo "Bounding box for \""$FILE"\" is: "$bbox

  # Save the old version of the file
  mv $FILE $BAK

  # Create the new version, replacing the old BoundingBox
  awk "$AWKPROG" $BAK > $FILE

  case `uname` in 
    "OS/2") dos2unix $FILE ;;
  esac

  # delete the backup file
  rm -f $BAK

done

